Efficient Active Learning of Halfspaces: an Aggressive Approach

We study pool-based active learning of half-spaces. We revisit the aggressive approach for active learning in the realizable case, and show that it can be made efficient and practical, while also having theoretical guarantees under reasonable assumptions. We further show, both theoretically and experimentally, that it can be preferable to mellow approaches. Our efficient aggressive active learner of half-spaces has formal approximation guarantees that hold when the pool is separable with a margin. While our analysis is focused on the realizable setting, we show that a simple heuristic allows using the same algorithm successfully for pools with low error as well. We further compare the aggressive approach to the mellow approach, and prove that there are cases in which the aggressive approach results in significantly better label complexity compared to the mellow approach. We demonstrate experimentally that substantial improvements in label complexity can be achieved using the aggressive approach, for both realizable and low-error settings.

==> experiments_ag.tex <==

\subsection{Experiments - agnostic case}
We tested the performance of ALuMA in the agnostic case while
comparing it to IWAL (see \cite{IWAL}) which is considered a state of
the art active learning algorithm for the agnostic case. As a first
experiment, we have generated a training set and a test set of size
$2000$ each of the pair $4,7$ of MNIST and reduced its
dimension from $784$ into $25$. Then, we used our preprocessing
technique and finally transformed the data into a separable data in
$\reals^{120}$. The noise parameter is $H = 10^{-2}$.  For IWAL, the
only parameter should be tuned is the norm of the candidate
hypotheses. We set it to $\sqrt{1000}$. We have also compared the two
algorithms to the passive soft-SVM algorithm. We set the
regularization parameter of soft-SVM to $\lambda=10^{-3}$
\alon{TODO: discuss why we have chosen these parameters}. This
parameter is also used when ALuMA calls soft-SVM to calculate the test
loss.The results
are shown in \figref{fig:MNIST47_ag_test} and \figref{fig:MNIST47_ag_train}.


\begin{figure}
\centering
\includegraphics[width = \textwidth]{MNIST47_test_ag.pdf}
\caption{MNIST 4 vs. 7. (non-separable, test).}
\label{fig:MNIST47_ag_test}
\end{figure}

\begin{figure}
\centering
\includegraphics[width = \textwidth]{MNIST47_train_ag.pdf}
\caption{MNIST 4 vs. 7. (non-separable, train).}
\label{fig:MNIST47_ag_train}
\end{figure}

Next, we performed a simillar experiment on the pair $3,5$ of MNIST (this time,
the train and the test consist of $1900$ instances each. The
parameters are identical). The results
are shown in \figref{fig:MNIST35_ag_test} and \figref{fig:MNIST35_ag_train}.


\begin{figure}[bth!] 
\centering
\caption{MNIST 3 vs. 5. (non-separable, test).}
\begin{tabular}{c}
\includegraphics[width = \textwidth]{MNIST35_test_ag.pdf}
\end{tabular}
\label{fig:MNIST35_ag_test}
\end{figure}

\begin{figure}[bth!] 
\centering
\caption{MNIST 3 vs. 5. (non-separable, train).}
\begin{tabular}{c}
\includegraphics[width = \textwidth]{MNIST35_train_ag.pdf}
\end{tabular}
\label{fig:MNIST35_ag_train}
\end{figure}

Finally, we performed an experiment over the CCAT data set
\alon{todo:cite and describe the data-set}. The original data contains
a (sparse representation of) more than $80000$ instances in
$\reals^{47236}$. We took a random subset of size $4,000$ and reduced
its dimension into $\reals^{700}$. Using our preprocessing
technique we finally transformed the data into a separable data in
$\reals^{600}$. The other parameters were chosen identically to the
previous experiments. The results are shown in \figref{fig:ccat_ag_test} and \figref{fig:ccat_ag_train}. 

\begin{figure}[bth!] 
\centering
\caption{CCAT (non-separable, test).}
\begin{tabular}{c}
\includegraphics[width = \textwidth]{ccat_test_ag.pdf}
\end{tabular}
\label{fig:ccat_ag_test}
\end{figure}

\begin{figure}[bth!] 
\centering
\caption{CCAT (non-separable, train).}
\begin{tabular}{c}
\includegraphics[width = \textwidth]{ccat_train_ag.pdf}
\end{tabular}
\label{fig:ccat_ag_train}
\end{figure}

As we can see from the results of the
passive soft-SVM algorithm, the CCAT dataset is noisier than the pair
$(3,5)$ which is noisier than the pair $(4,7)$. \alon{discuss further
  the influence of the noise on the performance of ALuMA and IWAL}.














%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ALuMA"
%%% End: 

















